Spatial Token Interleaving and Two-Pass BP Decoding for Semantic Image Transmission

Semantic error control coding (SECC) can correct the residual errors of a standard channel code with a foundation model that supplies a prior on the source content, but existing SECC schemes are designed for text. In this paper, we develop SECC for image transmission with spatial token interleaving and a two-pass belief propagation (BP) schedule. At the transmitter, a vector-quantized (VQ) tokenizer converts an image into tokens, which are transmitted in multiple low-density parity-check (LDPC) code blocks of fifth-generation New Radio (5G NR). In raster order, a block that BP fails to decode corrupts consecutive token rows, so the interleaver reorders the tokens such that adjacent tokens are carried by different blocks, without additional transmitted bits. At the receiver, after the first BP pass, token recovery fuses the token probabilities given by BP with the predictions of the autoregressive model Emu3-Gen, and the second BP pass decodes each block again with the fused distributions as priors on the information bits. On Kodak24 at 0.5 channel uses per pixel and a signal-to-noise ratio (SNR) of 0.15 dB, the second pass removes 92% of the token errors left by token recovery, and interleaving reduces the final token error rate by 88%. At medium to high SNR, the proposed receiver exceeds deep joint source--channel coding baselines with the same channel uses by at least 1.2 dB in peak signal-to-noise ratio.

==> figures/tikz/fig_decoder-integration.tex <==
% Preamble: \usepackage{amsmath,graphicx,tikz}
%           \usetikzlibrary{arrows.meta}
% Compile from the manuscript root so the thumbnail path resolves.
\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{\input{figures/tikz/fig_decoder}}
\caption{Visual decoder design. The $B$ block-wise APP LLR vectors are regrouped into $T$ token-wise vectors without changing the LLR order, then passed through the token deinterleaver. Coloured cells track the same LLRs across grouping boundaries; displayed group sizes are illustrative. The dashed loop appends each recovered token to the AR prefix for the next position.}
\label{fig:decoder-design}
\end{figure}


==> figures/tikz/fig_emu3-integration.tex <==
% Preamble: \usepackage{amsmath,amssymb,graphicx,tikz}
%           \usetikzlibrary{arrows.meta}
% Insert into the Emu3 token scoring subsection; compile from manuscript root.
\begin{figure}[!t]
\normalcolor
\centering
\resizebox{\columnwidth}{!}{\input{figures/tikz/fig_emu3}}
\caption{Emu3 token scoring at position $t$. The complete hard token sequence
$\tilde{\mathbf s}$ and the recovered prefix $\hat{\mathbf s}_{<t}$ jointly
condition the prediction of $s_t$. The amber input cell marks the observation
at the current position. Purple dashed arrows supply decisions recovered at
preceding positions. Softmax normalizes the model logits over the $V$
codebook candidates; the resulting probabilities are used in subsequent
BP--Emu3 score fusion. Probability bar heights are illustrative. The prefix
is empty at $t=1$. Ellipses omit intermediate tokens or candidates, and
sequence-formatting tokens are not shown.}
\label{fig:emu3-integration}
\end{figure}


==> figures/tikz/fig_encoder-integration.tex <==
% Packages in the manuscript preamble:
% \usepackage{amsmath,graphicx,tikz}
% \usetikzlibrary{arrows.meta}
% Compile from the manuscript root so the thumbnail path resolves.
\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{\input{figures/tikz/fig_encoder}}
\caption{Visual encoder design: Emu3 VQ tokenisation, interleaving and binary mapping into information blocks. The image grid and displayed token/bit segments are schematic.}
\label{fig:encoder-design}
\end{figure}


==> figures/tikz/fig_system-body.tex <==
% Compatibility entry point; edit fig_system.tex for the actual drawing.
\input{figures/tikz/fig_system}%


==> figures/tikz/fig_system-integration.tex <==
% Direct single-column TikZ inclusion; no precompiled PDF is required.
% Add to the manuscript preamble:
% \usepackage{amsmath,amssymb,graphicx,tikz}
% \usetikzlibrary{arrows.meta}
\begin{figure}[!t]
\centering
\input{figures/tikz/fig_system}%
\caption{System overview. The visual encoder supplies information blocks
$\mathbf u_j$ for LDPC encoding and BPSK transmission over AWGN. Soft
demodulation and BP decoding produce information-bit APP LLRs for the visual
decoder to reconstruct $\hat{\mathbf X}$. The visual encoder and decoder include token
interleaving and receiver-side recovery, respectively, as described in the text.
Small squares illustrate the transmitted and received symbol sequences.}
\label{fig:system}
\end{figure}

